Towards High-Quality Temporal Action Detection with Sparse Proposals

Temporal Action Detection (TAD) is an essential and challenging topic in video understanding, aiming to localize the temporal segments containing human action instances and predict the action categories. The previous works greatly rely upon dense candidates either by designing varying anchors or enumerating all the combinations of boundaries on video sequences; therefore, they are related to complicated pipelines and sensitive hand-crafted designs. Recently, with the resurgence of Transformer, query-based methods have tended to become the rising solutions for their simplicity and flexibility. However, there still exists a performance gap between query-based methods and well-established methods. In this paper, we identify the main challenge lies in the large variants of action duration and the ambiguous boundaries for short action instances; nevertheless, quadratic-computational global attention prevents query-based methods to build multi-scale feature maps. Towards high-quality temporal action detection, we introduce Sparse Proposals to interact with the hierarchical features. In our method, named SP-TAD, each proposal attends to a local segment feature in the temporal feature pyramid. The local interaction enables utilization of high-resolution features to preserve action instances details. Extensive experiments demonstrate the effectiveness of our method, especially under high tIoU thresholds. E.g., we achieve the state-of-the-art performance on THUMOS14 (45.7% on mAP@0.6, 33.4% on mAP@0.7 and 53.5% on mAP@Avg) and competitive results on ActivityNet-1.3 (32.99% on mAP@Avg). Code will be made available at https://github.com/wjn922/SP-TAD.

==> tables/ab_nms_anet.tex <==
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}
{c c c c c}
\toprule
Soft-NMS & 0.5 & 0.75 & 0.95 & Avg \\
\midrule
 & 46.88 & \textbf{33.07} & \textbf{8.60} & 32.28 \\
\checkmark & \textbf{50.06} & 32.92 & 8.44 & \textbf{32.99} \\
\bottomrule
\end{tabular}

==> tables/ab_nms_thumos.tex <==
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}
{c c c c c c c}
\toprule
Soft-NMS & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & Avg \\
\midrule
 & 62.8 & 58.7 & 52.4 & 43.4 & 32.0 & 49.9 \\
\checkmark & \textbf{69.2} & \textbf{63.3} & \textbf{55.9} & \textbf{45.7} & \textbf{33.4} & \textbf{53.5} \\
\bottomrule
\end{tabular}

==> tables/ab_pro.tex <==
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}
{c c c c c c c}
\toprule
Proposals & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & Avg \\
\midrule
10 & 67.7 & 61.4 &53.1 & 43.5 & 32.3 & 51.6 \\
30 & 66.2 & 61.1 & 53.3 & 42.2 & 32.5 & 51.1 \\
50 & \textbf{69.2} & \textbf{63.3} & \textbf{55.9} & \textbf{45.7} & \textbf{33.4} & \textbf{53.5} \\
70 & 68.1 & 63.4 & 55.8 & 44.7 & 33.5 & 53.1 \\
\bottomrule
\end{tabular}
